Securing Immersive 360 Video Streams through Attribute-Based Selective Encryption

Delivering high-quality, secure 360{\deg} video content introduces unique challenges, primarily due to the high bitrates and interactive demands of immersive media. Traditional HTTPS-based methods, although widely used, face limitations in computational efficiency and scalability when securing these high-resolution streams. To address these issues, this paper proposes a novel framework integrating Attribute-Based Encryption (ABE) with selective encryption techniques tailored specifically for tiled 360{\deg} video streaming. Our approach employs selective encryption of frames at varying levels to reduce computational overhead while ensuring robust protection against unauthorized access. Moreover, we explore viewport-adaptive encryption, dynamically encrypting more frames within tiles occupying larger portions of the viewer's field of view. This targeted method significantly enhances security in critical viewing areas without unnecessary overhead in peripheral regions. We deploy and evaluate our proposed approach using the CloudLab testbed, comparing its performance against traditional HTTPS streaming. Experimental results demonstrate that our ABE-based model achieves reduced computational load on intermediate caches, improves cache hit rates, and maintains comparable visual quality to HTTPS, as assessed by Video Multimethod Assessment Fusion (VMAF).

==> 5-related.tex <==
% \vspace{-1em}
% \section{Related Work} \label{sec:related}
% \textbf{ABE for video streaming:} 
% Prior works have utilized Attribute-Based Encryption (ABE) in the context of DASH video streaming \cite{10.1007/978-3-319-32689-4_26} and media clouds~\cite{doi:10.1177/1550147720908196}.
% %whereas \cite{doi:10.1177/1550147720908196} utilized ABE for media clouds. 
% However, these approaches employ ABE indirectly. They utilize AES to encrypt video content and ABE to encrypt and manage the AES keys. Evaluations in such approaches typically focus on encryption times for securing the AES key while varying the number of attributes in the ABE scheme.

% However, this method has several drawbacks, primarily the reuse of the same AES key for encryption and decryption. It requires managing two keys: the AES key for content encryption and the ABE key for AES key protection. If the AES key is compromised, the ABE scheme becomes ineffective. Additionally, revoking user access requires re-encrypting all content with a new AES key and redistributing it, which is inefficient.

% In contrast, our work applies ABE directly to the video segments, eliminating the need for a secondary AES key and simplifying key management. This approach avoids exposing the master key, as each user is issued a private key based on their access attributes. 
% % addressing the drawbacks of the previous method. 
% Content providers can use time-based ABE keys, requiring users to retrieve new keys periodically. This allows for easy revocation of access by excluding specific attributes from a user’s key without needing to re-encrypt content or affect other users. For example, 4K access can be revoked for all basic plan users while retaining it for premium users. This approach ensures uninterrupted access for authorized users while effectively revoking permissions for others. This method enhances security, simplifies key management, and provides flexible, attribute-based access control.


% \textbf{Caching for video delivery} For video delivery, existing caching solutions fall broadly into two categories. In the first category, the algorithms exploit the sequential access patterns of video segments to make better caching decisions. For example, CoLeap \cite{shi2020coleap} describes a pre-fetching-based cache algorithm that uses a QoE-oriented deep neural network model to decide the content to pre-fetch into the cache. Whereas \cite{10.5555/AAI28544902} proposes performing smart prefetching by forecasting throughput values in the cache using previous client throughput data, thus optimizing resource utilization by pre-fetching video segments based on predicted demand, while improving client QoE. Another approach, presented in \cite{10.1145/2713168.2713181}, introduces an integrated pre-fetching and caching proxy (ipac), a novel 0.5-competitive online pre-fetching algorithm specifically designed for HTTP-based adaptive streaming services like Netflix and YouTube, without requiring modifications to content servers or clients that improves byte-hit ratios and video rates.
% % The work in \cite{maniotis2021tile} employs Long Short-Term Memory (LSTM) networks to forecast the evolution of the content requests and pre-fetch content to caches for 360$^\circ$ video live streaming. 
% In the second category, the cache algorithms make decisions about specific qualities of each video segment to cache to maximize the cache hitrate for a single as well as a network of caches \cite{poularakis2016caching,  araldo2016representation}. 
% % Similarly, there exist several works \cite{lu2019transcoding, maniotis2019tile, zhang2020edge} that find the tiles of 360$^\circ$ to cache based on their popularity, size, quality, and their probability of being in the field of view of a viewer. 
% These approaches are orthogonal to \acro, which does not focus on admission and eviction strategies for video caching. Since \acro is agnostic to these strategies, any of them can be integrated in the streaming system we propose.


% % A recent work \cite{zhang2021video} proposes VISCA, VIdeo Super-resolution and Caching, a system that uses super-resolution and caching at the edge-server to serve end user requests faster. VISCA super-resolves the low-quality content that is cached in order to serve the request. Further, VISCA also proposes an adaptive bitrate algorithm (ABR) that runs on the edge server which decides the quality of content that needs to be served to the end user. While VISCA seems very close to our work, there are many differences. Firstly, the current HTTP multimedia protocols used in real systems expect the ABR algorithm to run on an end-user machine and not on the edge-server. We believe VISCA cannot be easily integrated into existing multimedia delivery systems, whereas \sysname provides seamless integration. Secondly, apart from super-resolution we also equip the edge-server to perform down-sampling or serve media content that is available in other qualities than the requested quality from within the cache. We believe this further reduces the mid-gress traffic as compared to VISCA. Thirdly, VISCA reports a best super-resolution speed of 40fps which means it takes 600ms to super-resolve a 1-second video encoded at 24fps. We believe this is too slow to provide real time video streaming. On the other hand, by using micromodels for super-resolution, \sysname can super-resolve up to 250 to 300fps. Thus, for the above reasons, we believe \sysname is more suitable to be deployed in multimedia delivery systems as compared to VISCA.\\



% %This work is based on earlier work~\cite{SabnisInfocom2021}

% %LRU is cost agnostic. It only looks at popularity and not of the cost of bringing something into the cached.
% %Work on cost-based eviction. 



==> 6-discussion.tex <==
%\vspace{-1em}
\section{Discussion} \label{sec:dicsussion}

Our experimental evaluation demonstrates that HTTP-based ABE streaming provides a compelling alternative to traditional HTTPS in 360-degree tiled video delivery. Across both small-scale and large-scale setups, ABE approaches consistently achieve lower CPU usage at caches, better hit rates, and comparable client-side QoE (VMAF). Notably, the ABE-allI+P scheme showed the best overall efficiency, outperforming ABE-MajorP in terms of CPU usage and hit rates due to its uniform encryption strategy.

A particularly interesting trend emerged in the small-scale experiment: as we reduced segment duration from 4 seconds to 2 seconds, the performance gap between HTTP-ABE and HTTPS widened. While HTTPS experienced increased CPU load and reduced hit rates—owing to more frequent TLS termination, decryption, and re-encryption operations—the ABE approaches maintained consistent performance. This suggests that ABE becomes increasingly efficient as segment granularity decreases, making it especially well-suited for applications with shorter segment durations.

This observation has important implications for live streaming, where segment durations are typically even smaller (e.g., 1–2 seconds) and scalability is critical. In such scenarios, HTTPS requires caches to terminate TLS sessions and re-encrypt segments for every client request, introducing substantial overhead. In contrast, ABE enables the cache to serve the same encrypted segment to multiple clients without any cryptographic processing, significantly improving scalability and reducing computational burden. This property of ABE makes it a promising candidate for large-scale, low-latency live video streaming, where performance and resource efficiency are paramount.

























% In our streaming experiments, the highest quality bitrate used  was 1920×1080 (FHD) at 5000 kbps. While FHD is common, modern services increasingly support higher resolutions such as 2K and 4K. Our Future work will include these higher-quality formats to align with advanced streaming practices.

% %Our experiments demonstrate that HTTP-ABE significantly reduces cache CPU usage compared to HTTPS while maintaining similar midgress traffic, cache hit rates, and QoE metrics. For higher-quality videos (e.g., 2K, 4K), we would proportionally adjust the server-cache bandwidth limit relative to the highest video bitrate, as we did for FHD (one-third of total bandwidth).

% Our experiments show that HTTP-ABE significantly lowers cache CPU usage compared to HTTPS while maintaining similar midgress traffic, cache hit rates, and QoE metrics. For higher-quality videos (e.g., 2K, 4K), we would adjust the server-cache bandwidth limit proportionally to the highest video bitrate, as done for FHD (one-third of total bandwidth).

% In this scenario, the CPU usage gap between HTTP-ABE and HTTPS would likely widen with higher bitrates. HTTPS requires TLS termination and re-encryption at the cache, which becomes more CPU-intensive for larger video segments. HTTP-ABE, by offloading encryption, reduces cache computational load, a benefit that scales with higher resolutions.

% % Regarding midgress traffic, cache hit rates, and QoE metrics, our results suggest that these factors would remain largely unchanged even with higher resolutions. In both our bandwidth-limited (Sec.~\ref{subsubsec:smallscaleexp} \& Sec.~\ref{subsubsec:large-scaleexp}) and non-limited experiment (Sec.~\ref{subsubsec:noBWlim}), these metrics showed no significant differences. Therefore, while increasing video quality to 2K or 4K would raise the overall bitrate, it is unlikely to have a major impact on these metrics, similar to what we observed with FHD.

% Midgress traffic, cache hit rates, and QoE metrics are expected to remain largely unchanged even at higher resolutions, similar to as observed in bandwidth-limited (Sec.~\ref{subsubsec:smallscaleexp} \& ~\ref{subsubsec:large-scaleexp}) and non-limited experiments (Sec.~\ref{subsubsec:noBWlim}). Thus, while improving quality will increase bitrate and bandwidth usage, the performance difference between HTTP-ABE and HTTPS is unlikely to change significantly.

%Thus, improve quality would increase bitrate and overall bandwidth consumption, the relative performance difference between HTTP-ABE and HTTPS is unlikely to be significantly affected.


% \textbf{Partial Encryption of video streams} has been widely researched in multimedia, offering various computational benefits \cite{10.5555/2907329.2907483}. Partial encryption can also offer privacy protection while maintaining the visibility of other parts of the video, like faces. For example, one approach \cite{8305040} encrypts faces in H.264 videos using object recognition to detect and track faces, allowing fine-grained control over encryption. Another study \cite{10.1145/3083187.3083192} combines face detection with AES encryption to blur faces while preserving original content. These methods could be enhanced with Attribute-Based Encryption (ABE), enabling selective decryption based on user attributes. For instance, in a kindergarten video, children’s faces could be encrypted for parental access, or courtroom footage could blur witness faces, allowing authorized individuals to decrypt them as needed.


%Work in\cite{reddick2022wip} explored ABE to provide access control in genomics data. It uses Named Data Networking (NDN) with attribute-based encryption and a timing attribute to invalidate the keys. This approach automates data invalidation, simplifies key management, and enables flexible, time-based access control without requiring continuous involvement from data publishers.

% \textbf{Multicasting for Live Streaming.}
% While the work presented in this paper primarily focuses on on-demand video streaming, there are also potential benefits for live streaming. Today's approaches for live streaming mostly depend on CDNs, which provide a multicast overlay (compared to on-demand, portions of the live stream will only briefly buffered at edge servers). In the case of live streaming, \acro will increase its efficiency and scalability since it eliminates the requirement for TLS termination. This could have an important impact on reducing latency since no decryption and encryption has to be performed at the cache. This is a critical aspect for a low-latency application like live streaming. We will further investigate the benefits of \acro in the case of live streaming in future work.


% \textbf{Caching Hierarchies}
% In traditional caching hierarchies, TLS termination requires cumulative encryption and decryption operations at each cache, which can introduce significant latency due to the repeated processing at every cache level. By minimizing these operations, \acro can improve the overall latency and efficiency of content delivery in systems that utilize caching hierarchies. Further, data is secured at rest, reducing the need to track caching endpoints. From a CDN's perspective, this can reduce the number of TLS terminations required.

% \textbf{Implications for AR/VR}
% Augmented Reality (AR) and Virtual Reality (VR) applications present unique challenges due to the substantial data volumes involved, especially when compared to standard video streaming. For instance, 360-degree video with equirectangular projection generates multiple individual video streams, each corresponding to a specific tile in the projection. Therefore, an efficient encryption strategy becomes critical in this large-data context. \acro's ability to reduce encryption overhead can significantly improve performance for AR/VR streaming, which is highly sensitive to bandwidth and latency variations.

% \textbf{Compatibility with Existing Systems}
% The proposed approach is fully compliant with the DASH standard, allowing it to function independently of any particular bitrate adaptation algorithm. This flexibility ensures broad applicability in existing streaming infrastructures that leverage DASH. It is also fully compliant with existing content delivery networks, which means it can be deployed for content delivery immediately with a little modification required on the DASH streaming client to handle.
% \textbf{Adapting the Principles of Content-Centric Networking (CCN)}
% \acro also aligns with Content-Centric Networking (CCN) principles, wherein content is delivered based on its named identity rather than the host's location. By optimizing encryption and cache operations, \acro can contribute to the growing field of CCN, improving the scalability and efficiency of content distribution networks. 
% \textbf{Open Source Availability}
%  To foster further research and development, we intend to release all relevant code and resources as open-source. This approach will allow other researchers and developers to build upon our work and apply it in various domains.
